Differentially-Private "Draw and Discard" Machine Learning

In this work, we propose a novel framework for privacy-preserving client-distributed machine learning. It is motivated by the desire to achieve differential privacy guarantees in the local model of privacy in a way that satisfies all systems constraints using asynchronous client-server communication and provides attractive model learning properties. We call it "Draw and Discard" because it relies on random sampling of models for load distribution (scalability), which also provides additional server-side privacy protections and improved model quality through averaging. We present the mechanics of client and server components of "Draw and Discard" and demonstrate how the framework can be applied to learning Generalized Linear models. We then analyze the privacy guarantees provided by our approach against several types of adversaries and showcase experimental results that provide evidence for the framework's viability in practical deployments.

==> old_amplification_proofs.tex <==
%\subsection{Proofs of Privacy Amplification Lemmas from Section~\ref{sec:privacy-subpoena}}\label{sec:amp-proofs}

\iffalse
\begin{proof}[\textbf{Proof of Lemma~\ref{lem:pamp-draw}}]
Let $a$ and $a'$ denote the two possible values of the client's data. We are interested in bounding $P[(B_1^{t+1}, \ldots, B_k^{t+1}) | a] / P[(B_1^{t+1}, \ldots, B_k^{t+1}) | a']$, where we assume that $(B_1^{t+1}, \ldots, B_k^{t+1})$ are obtained from $(B_1^{t}, \ldots, B_k^{t})$ after the client's update given their data was $a$ or $a'$ respectively. As per our adversary model, he doesn't have access to $\textbf{B}^{t}$, only to $\textbf{B}^{t+1}$, but he knows the process by which $\textbf{B}^{t+1}$ is obtained from $\textbf{B}^{t}.$ 

Let $B_i^t$ be the model sent to the client by the ``Draw step", and let $B^*$ be the model returned by the client. One can consider two distinct situations: 1) in the ``Discard" step, $B_i^t$ is chosen to be discarded, and thus $B_i^{t+1}$ becomes $B^*$; 2) in the ``Discard" step, some other model instance $j$ is chosen to be discarded, and thus $B_j^{t+1} = B^*$. Denote $(B_1^{t+1}, \ldots, B_k^{t+1})$ by $\textbf{B}_{i,i}$ for case 1) and $\textbf{B}_{i,j}$ for case 2).

Observe that $P[\textbf{B}_{i,i} | a, i \leftarrow i] = P[\textbf{B}_{i,i} | a', i \leftarrow i]$, since $B^*$ is equally likely whether the data was $a$ or $a'$ in the absence of other information.

Observe that $\frac{P[\textbf{B}_{i,j} | a, j \leftarrow i]}{P[\textbf{B}_{i,j} | a', j \leftarrow i]} \leq \exp(\epsilon),$ by local differential privacy of Section~\ref{sec:privacy-local}. In fact, this is the worst-case upper bound. In practice, the adversary doesn't know which $i$ was the ``pre-image" of the $j$-th model instance at time $t+1$, and there may be multiple such $i$s.

\scriptsize
\[P[\textbf{B} | a] = \sum_{i} (P[\textbf{B} | a, i \leftarrow i] \cdot P[i \leftarrow i] + \sum_{j, j \neq i} P[\textbf{B} | a, j \leftarrow i] \cdot P[j \leftarrow i]) = \]
\[= \frac{1}{k^2} \sum_{i}P[\textbf{B} | a, i \leftarrow i] + \frac{k-1}{k^2} \sum_{i,j, j \neq i} P[\textbf{B} | a, j \leftarrow i] \leq \]
\[\leq \frac{1}{k^2} \sum_{i}P[\textbf{B} | a', i \leftarrow i] + \frac{k-1}{k^2} \exp(\epsilon) \sum_{i,j, j \neq i} P[\textbf{B} | a', j \leftarrow i] = \]
\[= \exp(\epsilon) P[\textbf{B} | a'] -  \frac{1}{k^2} \sum_{i}P[\textbf{B} | a', i \leftarrow i] \left(\exp(\epsilon) -1 \right) \]
%\[= \exp(\epsilon) P[\textbf{B} | a'] - \frac{1}{k} (\exp(\epsilon)-1) \]
\normalsize

Hence, $\frac{P[\textbf{B} | a]}{P[\textbf{B} | a']} \leq 
\exp(\epsilon) - \frac{\frac{1}{k^2} \sum_{i}P[\textbf{B} | a', i \leftarrow i] \left(\exp(\epsilon) -1 \right)}{P[\textbf{B} | a']} \leq $

\TODO{How to simplify next? Desired goal $\exp(\epsilon) - \frac{1}{k} (\exp(\epsilon)-1) $}

$
\exp(\epsilon) - \frac{1}{k^2} \sum_{i}P[\textbf{B} | a', i \leftarrow i] \left(\exp(\epsilon) -1 \right)
$.

%$P[\textbf{B} | a, j \leftarrow i]  = P[B_i^{t+1}=B^* | a, B_i] \leq \exp(\epsilon) P[B_i^{t+1}=B^* | a', B_i] $ 


%and let $B^*$ denote \TODO{a model corresponding to the client's update}. In the first case, $P[B^* | a ] = P[B^* | a']$. In the second case, suppose the adversary knows exactly which model $B_i$ is the pre-image of the model $B^*$. By local differential privacy $\frac{P[B^* | B_i, a]}{P[B^* | B_i, a']} \leq \exp(\epsilon)$.
%Therefore, $\frac{P[B^* | a]}{P[B^* | a']} = \frac{P[B^* | a, B_i] \cdot Pr[preimage is B_i] + P[B^* | a, no known pre-image] \cdot P[no known preimage]}{P[B^* | a']} \leq \frac{k-1}{k} \frac{P[B^* | B_i, a]}{P[B^* | B_i, a']}$
\end{proof}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{proof}[Vasyl's old Proof]
%Assume we have $k$ models and add Laplace noise with scale $2\gamma / \epsilon$ on the client side. Let $B^*$ be the updated value of the model and $B$ the original. 
%\begin{eqnarray*}
%&&R \\
%&=& \frac{P(B^* = b^*, B = b | X = 1, Y = 1)}{P(B^* = b^*, B = b | X = 1, Y = 0)} \\
%&=& \frac{P(B^* = b^* | X = 1, Y = 1, B = b) P(b) + P(B^* = b^* | B = b') P(b')}{P(B^* = b^* | X = 1, Y = 0, B = b) P(b) + P(B^* = b^* | B = b') P(b')} \\
%&=& \frac{e^{-\frac{\epsilon|b^* - \gamma|}{2\gamma}}\frac{k-1}{k} + 1 * \frac{1}{k}}{e^{-\frac{\epsilon|b^* + \gamma|}{2\gamma}}\frac{k-1}{k} + 1 * \frac{1}{k}} \\
%&=& \frac{(k-1)e^{-\frac{\epsilon|b^* - \gamma|}{2\gamma}} + 1}{(k-1)e^{-\frac{\epsilon|b^* + \gamma|}{2\gamma}} + 1} \\
%&<& \frac{e^{-\frac{\epsilon|b^* - \gamma|}{2\gamma}}}{e^{-\frac{\epsilon|b^* + \gamma|}{2\gamma}}} \\
%&=& e^{\epsilon}.
%\end{eqnarray*}
%
%Here, $b'$ is the model that got replaced (one of the $k$ whose values we assume to support $Y$ and $X$). This model completely supports $B^*$; therefore, its probability is 1. 
%
%The savings in privacy are quite significant. Privacy gets worse as $k$ increases (which makes sense since we store more data on the server-side). For relatively small $k$ ~100, the $R$ is cut in about a half.
%\end{proof}

%Need to prove that each individual update preserves $\epsilon$ or $(\epsilon, \delta)$ differential privacy in the local model (Section~\ref{sec:related-local}). For that, need to see the relationship between clipping of the gradient, sensitivity, $\eta$, in our algorithm (see \cite{Abadi2016} page 3 for example of how it's done).




%\begin{proof}[\textbf{Proof of Lemma~\ref{lem:symmetry}}]
%The intuition for the proof is as follows: if the adversary doesn't know which of the $k$ models corresponds to $B^*$, then, by design of DDML, he has to assume that each of the models is equally likely to be $B^*$. Then, whenever one has two models, $B_i$ and $B_j$, assuming that $B_i$ is the pre-image of $B_j$ gives the same support for $a$ as the support that assuming that $B_j$ is the pre-image of $B_i$ gives for $a'$. 
%
%%More precisely, $\frac{P[B_i | B_j, a]}{P[B_i | B_j, a']} =  \frac{\exp(-\frac{\epsilon}{2\gamma} |b_i-b_j+\gamma \cdot a|)}{\exp(-\frac{\epsilon}{2\gamma} |b_i-b_j+\gamma \cdot a'|)} $ and
%%
%%$\frac{P[B_j | B_i, a]}{P[B_j | B_i, a']} = \frac{\exp(-\frac{\epsilon}{2\gamma} |b_j-b_i+\gamma \cdot a|)}{\exp(-\frac{\epsilon}{2\gamma} |b_j-b_i+\gamma \cdot a'|)} $.
%
%Therefore, the ``worst-case" scenario from the privacy guarantee perspective is when $\textbf{B}$ consists of $k$ identical models $B$. In that case, with probability $\frac{1}{k}$, the pre-image was lost, and its PDF is therefore, $\frac{\epsilon}{4 \gamma}$, or, with probability $\frac{k-1}{k}$, $B$ was the pre-image of $B$.
%\end{proof}

\subsubsection{Privacy Amplification due to ``Draw" and Variance Stabilization Resulting in Multiple Pre-image Candidates}\label{sec:multiple-preimages}

Consider the situation when the client knows that the pre-image of the model has not been discarded, but does not know which of the $k$ models is the pre-image. We observe that for any fixed $B^*$, if there are 2 pre-image candidates at most $t\gamma$ away from it ($0 < t <1$), then the lack of adversary II's knowledge which of these is the true pre-image further amplifies the privacy guarantee to $t\epsilon$.

\begin{lemma}\label{lem:distance}
If $B^*$ has 2 pre-images that are less than $t \gamma$ away from $B^*$ (no matter from which side), where $t<1$, then the privacy guarantee against adversary II becomes $\exp(\epsilon t)$, i.e., it improves by a factor of $t$.
\end{lemma}

\begin{figure}[b]
\centering
\includegraphics[width=0.45\textwidth]{imgs/delta-epsilon.pdf}
\caption{Empirical probability of updated model having less than 2 pre-images within $t\gamma$ for $\epsilon = 7$.}
\label{fig:k_vs_privacy}
\end{figure}

Figure~\ref{fig:k_vs_privacy} illustrates the implications of Lemma~\ref{lem:distance} by showing the empirically computed likelihood of $B^*$ having fewer than 2 candidate pre-images within $t \gamma$ for various choices of $k$ and $\gamma$. As expected, the higher the $k$, the more densely the images are distributed and, therefore, it is more likely that conditions of Lemma~\ref{lem:distance} hold.

An intuitive way to interpret this amplification is to say that for $k=60$, with probability 84.1\%, we have the privacy guarantee of $0.2\epsilon$ against Adversary II, and with probability 15.9\%, there is no additional privacy amplification. % and we have the same privacy guarantee as against Adversary I, of $\epsilon$.

Note that the analysis in Lemma~\ref{lem:distance} disregards the fact that our models have $p$ features each, as discussed in Section~\ref{sec:feature-level}.

\begin{proof}[\textbf{Proof of Lemma~\ref{lem:distance}}]
Let $b_1$ and $b_2$ be pre-image candidates for $b^*$. We use lowercase $b$ to reflect the fact that this Lemma is applied at the level of features (as discussed in Section~\ref{sec:feature-level}).

To prove DP, we are interested in bounding $R = \frac{P[b^*|a, b_1, b_2]}{P[b^*|a', b_1, b_2]} = \frac{P[b^*|a, b_1] + P[b^*|a, b_2]}{P[b^*|a', b_1] + P[b^*|a', b_2]},$ since $b_1$ and $b_2$ are equally likely to be pre-images due to the ``draw" of the DDML process.

Moreover, due to the noise addition and learning rate choice of DDML, the upper and lower bounds on $R$ are realized when the gradients are $-1$ and $1$. 
% \TODO{Needs proof}. 
Hence, 
$R = \frac{\exp(-\frac{\epsilon}{2\gamma} |b^*-b_1+\gamma|)+\exp(-\frac{\epsilon}{2\gamma} |b^*-b_2+\gamma |)}{\exp(-\frac{\epsilon}{2\gamma} |b^*-b_1-\gamma|)+\exp(-\frac{\epsilon}{2\gamma} |b^*-b_2-\gamma|)}$. % \aleks{We plugged in $\gamma, -\gamma$, but it's not clear it is truly wlog.} 

Wlog, we need to consider two scenarios: $b_2 \leq b_1 \leq b^*$ and $b_1 \leq b^* \leq b_2$.
Consider the first scenario first.

%Denote $b^*-b_1 = x$, $b_1-b_2 = \delta$, then $b^*-b_2=x +\delta$. 
Assume $b^*-b_1 < \gamma$ and $b^*-b_2 < \gamma$. Then

\[R =  \frac{\exp(-\frac{\epsilon}{2\gamma} (b^*-b_1+\gamma))+\exp(-\frac{\epsilon}{2\gamma} (b^*-b_2+\gamma))}{\exp(-\frac{\epsilon}{2\gamma} (-b^*+b_1+\gamma))+\exp(-\frac{\epsilon}{2\gamma} (-b^*+b_2+\gamma))}\]
\[ = \exp(-\frac{\epsilon b^*}{\gamma}) \cdot \frac{\exp(\frac{\epsilon}{2\gamma} b_1) + \exp(\frac{\epsilon}{2\gamma}b_2)}{\exp(-\frac{\epsilon}{2\gamma} b_1) + \exp(-\frac{\epsilon}{2\gamma} b_2)} \] 

\[\frac{1}{R} = \exp(\frac{\epsilon b^*}{\gamma}) \cdot \frac{\exp(-\frac{\epsilon}{2\gamma} b_1) + \exp(-\frac{\epsilon}{2\gamma}b_2)}{\exp(\frac{\epsilon}{2\gamma} b_1) + \exp(\frac{\epsilon}{2\gamma} b_2)} \leq \]

\[\leq \exp(\frac{\epsilon b^*}{\gamma}) \cdot \max (\exp(-\frac{\epsilon}{\gamma} b_1), \exp(-\frac{\epsilon}{\gamma} b_2)) = \exp(\frac{\epsilon}{\gamma} (b^*-b_2)) \] 


Consider the second scenario, $b_1 \leq b^* \leq b_2$.
Assume $b_2-b^* < \gamma$ and $b^*- b_1 < \gamma$. Then

\[R =  \frac{\exp(-\frac{\epsilon}{2\gamma} (b^*-b_1+\gamma))+\exp(-\frac{\epsilon}{2\gamma} (b^*-b_2+\gamma))}{\exp(-\frac{\epsilon}{2\gamma} (-b^*+b_1+\gamma))+\exp(-\frac{\epsilon}{2\gamma} (-b^*+b_2+\gamma))}\]
which is exactly the same expression as in the first scenario. Hence, 
$\frac{1}{R} \leq \exp(\frac{\epsilon b^*}{\gamma}) \cdot \max (\exp(-\frac{\epsilon}{\gamma} b_1), \exp(-\frac{\epsilon}{\gamma} b_2)) = \exp(\frac{\epsilon}{\gamma} (b^*-b_2)).$

The other scenarios are analogous.
\end{proof}


